Data-Efficiency with a Single GPU: An Exploration of Transfer Methods for Small Language Models

Multi-task learning (MTL), instruction tuning, and prompting have recently been shown to improve the generalizability of large language models to new tasks. However, the benefits of such methods are less well-documented in smaller language models, with some studies finding contradictory results. In this work, we explore and isolate the effects of (i) model size, (ii) general purpose MTL, (iii) in-domain MTL, (iv) instruction tuning, and (v) few-shot fine-tuning for models with fewer than 500 million parameters. Our experiments in the zero-shot setting demonstrate that models gain 31% relative improvement, on average, from general purpose MTL, with an additional 37.6% relative gain from in-domain MTL. Contradictory to prior works on large models, we find that instruction tuning provides a modest 2% performance improvement for small models.

==> sections/introduction.tex <==
\section{Introduction}

Many recent works have demonstrated the benefits of prompting for large language models (see \citet{prompt_survey} for an extensive survey). The utilization of prompts has further expanded into the use of demonstrations, examples, and task instructions, all of which have been shown to improve the generalization of language models to unseen tasks \citep{FLAN,Mishra2021NaturalIB,Ouyang2022TrainingLM}.

Studies on utilizing prompts have shown that as model sizes scale up, the generalization abilities of a model increase \citep{gpt3, lester-etal-2021-power,demonstrations_icl}. However, utilizing models on the hundred-billion parameter scale is not accessible for most researchers and practitioners. Furthermore, \citet{wei2022emergent} show that trends for large language models do not hold for smaller language models. 
For this reason, it is crucial that we must empirically find the trends that occur in smaller models and cannot rely on studies of larger models. Additionally, for situations with latency and memory limitations, small models may be the only option. In particular, we study zero- and few-shot performance on dialogue tasks, a sample domain in which reducing latency and memory usage are of high importance. 
% Additionally, some use cases for language models, such as conversational agents, may have strict requirements for memory and latency, reducing the possible use cases for advances in prompting methods.

Similar efforts have demonstrated the benefits of task instructions in the dialogue domain \citep{instructdial}. However, some findings have been contradictory across studies. For example, \citet{FLAN} found that models with fewer than 8B parameters see decreases in generalization capabilities when training with instructions, whereas \citet{instructdial} finds consistent gains in models with 3B and fewer parameters. To conflate these results further though, \citet{instructdial} only consider 2 situations: when inputs include prompts and instructions, or if inputs include no prompt and no instruction at all. 

Simultaneously with the emergence of prompting, the explicit multi-task learning (MTL) paradigm emerged, with works such as Muppet \citep{aghajanyan-etal-2021-muppet} or T0 \citep{sanh2022multitask} and their variants. Explicit MTL has been demonstrated as a means of improving the downstream performance of pre-trained language models in data-constrained settings.
% However, many prior studies of explicit MTL also do not consider models smaller than the billion parameter scale.
In this work we consider 2 types of MTL: general purpose and in-domain. Specifically, general purpose MTL consists of training across a wide variety of tasks and domains, whereas in-domain MTL consists of training across a variety of tasks that all occur within a domain. In this work, we focus on the dialogue domain.


In this work we bridge the gap between previous studies by exploring the effects of a variety of factors on the zero- and few-shot generalizability of modestly sized language models (<500M parameters). Specifically, we run experiments to find the effects of: (i) model size, (ii) general purpose MTL, (iii) in-domain MTL, and (iv) instruction tuning. Additionally, to better understand the sensitivity of models to instruction phrasing, we analyze variations in performance across task instructions.
For the few-shot setting, we additionally consider (v) the effects of fine-tuning with and without instructions.

% This work also analyses variations across task instructions used in zero-shot inference, and we find that instructions which deviate from natural language tend to lead to worse performance compared with instructions that use more standard language. For example, instructions that use the phrase <mask> prove detrimental to performance.

In this study, we find that
\textbf{(1)} In-domain multi-task learning (MTL) gives the largest improvements to generalizability, up to 80\% increased relative performance, and 37.6\% on average across all models
\textbf{(2)} Increasing model size alone has little effect on generalization, but when combined with in-domain MTL leads to double the (already strong) performance improvement of in-domain MTL
\textbf{(3)} General purpose MTL can provide large gains (57\% improvement) for downstream tasks which closely resemble the MTL tasks, but still provides modest gains (5\%) even for tasks which are more dissimilar
\textbf{(4)} Instruction tuning during in-domain MTL provides modest gains of just over 2\% performance, regardless of model size.
% \textbf{(5)} Instructions which deviate from natural language tend to lead to worse performance compared with instructions that use more standard language. For example, instructions that use the phrase "<mask>" prove detrimental to performance.
% \textbf{(5)} Instructions which utilize domain-specific wording see the best performance


% aa - Model size and in-domain MTL prove to be a strong combination of factors, leading to double the gains from in-domain MTL alone
% aa - in-domain MTL leads to up to 80\% improvement, and 37.6\% improvement on average.
% aa - general MTL leads to 57\% improvement on classification, but only 5\% for generation tasks (importance of matching the MTL tasks to downstream task)
% aa - instruction tuning during in-domain MTL on average provides modest gains (just over 2\% improvement)


==> sections/preliminaries.tex <==
% \section{Preliminaries}

% \paragraph{Why should we study small models?}
% Previous studies have shown that trends in large language models (>1B parameters) do not hold for smaller language models \citep{wei2022emergent}. For this reason, it is crucial that we must empirically find the trends that occur in smaller models and cannot rely on studies of larger models. Additionally, for situations with latency and memory limitations, small models may be the only option. In particular, we study zero- and few-shot performance on dialogue tasks, a sample domain in which reducing latency and memory usage are of high importance. 

% \paragraph{What are prompting methods?}
% In this study, we convert all tasks to a sequence-to-sequence format, allowing for a single generative model to perform all tasks \citep{2020t5}. By treating all tasks as sequence-to-sequence, we can also include textual prompts as part of the text input. In this work, we focus on two types of prompts: answer templates and instructions. First, \textbf{answer templates} are a string of text added to the end of the input sequence that specifies the task and which allows the model to solve the task by filling in the template in natural language \citep{prompt_survey}. This is in contrast to more simple prompts which only specify the task by including an identifier (eg. "cola sentence" for linguistic acceptability, or "topic" for topic classification) \citep{2020t5, FETA}. Second, we also consider \textbf{instructions}, which are generally added at the beginning of the input sequence and describe the task in natural language. For example, an instruction for document grounded generation is "Read the dialogue and the document text to generate a response."

% \paragraph{How is explicit multi-task learning (MTL) used?}
% Explicit MTL has emerged as a strong paradigm for eliciting zero-shot generalization in large language models \citep{sanh2022multitask}. In this work we consider 2 types of MTL: general purpose and in-domain. Specifically, general purpose MTL consists of training across a wide variety of tasks and domains, whereas in-domain MTL consists of training across a variety of tasks that all occur within a domain. In this work, we focus on the dialogue domain.
